On Testing Machine Learning Programs

Nowadays, we are witnessing a wide adoption of Machine learning (ML) models in many safety-critical systems, thanks to recent breakthroughs in deep learning and reinforcement learning. Many people are now interacting with systems based on ML every day, e.g., voice recognition systems used by virtual personal assistants like Amazon Alexa or Google Home. As the field of ML continues to grow, we are likely to witness transformative advances in a wide range of areas, from finance, energy, to health and transportation. Given this growing importance of ML-based systems in our daily life, it is becoming utterly important to ensure their reliability. Recently, software researchers have started adapting concepts from the software testing domain (e.g., code coverage, mutation testing, or property-based testing) to help ML engineers detect and correct faults in ML programs. This paper reviews current existing testing practices for ML programs. First, we identify and explain challenges that should be addressed when testing ML programs. Next, we report existing solutions found in the literature for testing ML programs. Finally, we identify gaps in the literature related to the testing of ML programs and make recommendations of future research directions for the scientific community. We hope that this comprehensive review of software testing practices will help ML engineers identify the right approach to improve the reliability of their ML-based systems. We also hope that the research community will act on our proposed research directions to advance the state of the art of testing for ML programs.

==> TheRoadAhead.tex <==
\section{The Road Ahead}\label{sec:road_ahead}
%\Foutse{here we should make sure to connect back to our figure and challenges and highlight what haven't be addressed yet by the literature so that we can make some recommendations for the community going forward!!!}
%\Foutse{we should recall the figure showing the multi-dimensional challenges of testing ML and discuss what is left to be done and where we want to see research going!!!}\\
Figure~\ref{x}\Foutse{figure to be added!} summarises the literature on ML program testing along the dimensions presented in Figure~\ref{fig:testing_space}. As one can see, very few research efforts have been dedicated to the detection of rounding errors in ML code implementations. \Foutse{we should list all the types of errors that have not been covered!} 
Regarding the approaches proposed to detect errors in data pipelines, they do not support the end to end development and deployment process of the ML program. Specific tests should be written to ensure that the data pipeline quality is not regressed over time due to unstable and epsilon features. The research community should consider devoting some effort to develop efficient testing techniques to help ML developers ensure quality in their feature engineering infrastructure. %during the overall deveWe recommend that the research community  have been mentioned in [ref]. Briefly recall unit tests and integration tests in software engineering.
For example, unit tests should be developed to help verify that data invariants hold in new or augmented training datasets. Unit tests are also needed to test that each transformer operation included in the data pipeline performs as expected. Integration tests are also needed to validate that a pipeline is working correctly, \ie{} it is providing well-represented features that can feed the model efficiently. These integration tests can also help ensure that each newly selected feature contributes significantly to the model, and %Moreover, at integration testing, the usefulness of each feature in terms of contribution to the predict output should be re-evaluated, so this makes sure of the utility of new features and there is
that none of the existing features have became obsolete. %in the model have became redundant. %loses its contribution because of information redundancies.

%testing, the white-box testing show prominent results and several coverage measures were invented in order to measure the proportion of learned logic that was solicited by the test data collected or generated. We have seen that for some coverage measures, we have reached 100\% coverage and for other multi-level measures, we have been able to know the different most active areas. Therefore, focusing on the automated generation of new data to cover the maximum of corner cases and teach the model different behaviors not learned\Foutse{to be completed!}. We should question the model architecture and the corresponding fixed hyperparameters. In fact, there is no theory in machine learning behind these different choices. As we have introduced in [section], a search-based algorithm tunes them to best define the accuracy obtained on the validation data.
%As a result, coverage measurement results should be used to change the hyperparameters in order to improve the ability of model learning to relate to the problem. The most telling example is the deep neural networks that require the fixation of many layers as well as the number of neurons per layer. The analysis of the neuronal coverage and the coverage of the different layers makes it possible to make specific changes in the model in the sense that we improve the ability of neural networks to identify the maximum of the relevant hidden patterns in order to recognize the most subtle behaviors.
%Concerning the implementation, end-to-end tests of ML systems are valuable, but in the face of a multiple sources of errors in such complex software system including scientific computations, global tests are not sufficient to provide evidence that a system is working as intended. U
%unit testing of individual components becomes a requirement when the ML code represents a real-world application that would be deployed in production. Unfortunately, the way machine learning algorithms are represented in white-papers and books enhances a programming style which is neither modular nor testable [ref]. Indeed, ML beginners typically first derive the update rules for an iterative algorithm, and then implement the updates directly. This approach makes it easy to spot differences from the correct solution, but it is not a robust way to build real software projects. Therefore,
%the code must be refactored in a modular way when it would be the core logic of in-production ML system, such that different chunks are independently testable.
%Recently, the evolution of advanced ML open source libraries such as medium-level [section] allows scientists to formulate ML algorithm in terms of general ML configurable routines that suggest a modular organization of the ML program. But as needs evolves, a lot of things get changed. Multiple models are tested, helper functions are added to process data, optimization algorithms and parameters are tried. As soon as the model is well fitted to the data, we decide to put it into production. Nevertheless, we end up with a spaghetti code as introduced in [section].
%To avoid this poor code quality that hinders testing and debugging, the code implementing the model engineering process must be maintainable, in other words, the code can be maintained in order to make maintenance and defect correction easier. Thus, author et al[ref] claim that it could be much easier to try to keep things modular and testable from the beginning. Moreover, it is necessary to detect code smells and anti-patterns occurring in those engineering ML projects in order to improve their comprehension and testability. This is the main lesson falls under the claim contained within the paper [ref] that is a result of hard-won experience at Google ``just because there’s machine learning involved it doesn’t mean you can forget good software engineering practices''.

Regarding the model, a component based architecture that allows testing components independently is likely to improve reliability. We recommend that the research community develop architectural methodologies to help ML developers architect their ML program in a modular way to allow for unit and integration testing. %unit testing of individual components and end-to-end tests of ML program during implementation phase are necessary, but in the face of a changing world such tests are not sufficient to provide evidence that the resulted ML system would run as intended in production. 
Post-deployment testing and system performance monitoring are also critical aspect to be investigated. First, the data pipeline that actually extracts input features may differ for training and deployment environments. It is therefore important to verify key invariants on both training and deployment environments, and test that serving features compute the same expected values as training features.  Second, it is important to test for numerical instabilities (i.e., NaNs and infinities) on models in-production (\ie{} as a post-deployment test), because the execution environment is likely to be different from the training environment. %, and, consequently, this can cause invalid numeric values.
Third, the system in-production should be monitored via specific regression testing in order to quickly identify, (i) any deterioration in terms of prediction quality on served data, and (ii) any degradation in terms of resources-consuming performance such as higher serving latency value or excessive RAM usage. These symptoms could indicate the occurrence of defects resulting from outside changes whether in served data or infrastructure.



